Efficient Approaches for GEMM Acceleration on Leading AI-Optimized FPGAs

FPGAs are a promising platform for accelerating Deep Learning (DL) applications, due to their high performance, low power consumption, and reconfigurability. Recently, the leading FPGA vendors have enhanced their architectures to more efficiently support the computational demands of DL workloads. However, the two most prominent AI-optimized FPGAs, i.e., AMD/Xilinx Versal ACAP and Intel Stratix 10 NX, employ significantly different architectural approaches. This paper presents novel systematic frameworks to optimize the performance of General Matrix Multiplication (GEMM), a fundamental operation in DL workloads, by exploiting the unique and distinct architectural characteristics of each FPGA. Our evaluation on GEMM workloads for int8 precision shows up to 77 and 68 TOPs (int8) throughput, with up to 0.94 and 1.35 TOPs/W energy efficiency for Versal VC1902 and Stratix 10 NX, respectively. This work provides insights and guidelines for optimizing GEMM-based applications on both platforms, while also delving into their programmability trade-offs and associated challenges.

==> Intel_Stratix/Stratix.tex <==

The Intel Stratix 10 NX 2100 device was quickly developed on top of the existing Stratix 10 MX 2100 architecture and replaces the traditional variable-precision DSP blocks with the AI-optimized Tensor blocks. The Tensor blocks drop many of the operating modes and functionalities of the DSP blocks and replace them with with scalar, vector and tensor operating modes for several data types. The resulting block interface is exactly the same as before, with a small change in area and power.
\subsection{Stratix 10 NX AI Tensor Block}


\begin{figure}[t]
\includegraphics[width=1.0\columnwidth]{Intel Stratix/tensor_block_diagram.pdf}
\caption{Tensor Block block diagram and example chain of 4 cascaded Tensor blocks. The first block in the chain operates in parallel load mode and does not perform any computation. Subsequent blocks operate in Tensor \texttt{int8} mode.}
\label{fig_tensor_block_diagram}
\end{figure}


\begin{figure*}[!t]
%\fbox{\includegraphics[width=1.0\textwidth]{Intel Stratix/tb_layout.pdf}}
\includegraphics[width=1.0\textwidth]{Intel Stratix/tb_layout.pdf}
\caption{Tensor Block layout. Shapes indicate what weights get stored in each Tensor block. Colors indicate the groups of input data that get multiplied with each Tensor block's weights. Numbers indicate what clock cycle each input data is multiplied with the corresponding weights.}
\label{fig_tb_layout}
\end{figure*}


\textcolor{red}{Missing: Explicitly talk about cascade/hard connections.} Figure \ref{fig_tensor_block_diagram} shows a simplified block diagram of the Tensor block and a Tensor block chain. A Tensor block supports many modes of operation, but here we focus on the one we use, i.e. the Tensor \texttt{int8} mode. Each block contains 2 sets of 3 ping-pong buffers each for the weights, where each buffer holds 10 8-bit values. It also has 3 dot product engines of length 10 each. The first input to each engine comes from its corresponding buffer, while the second input is broadcast from the 80-bit wide \texttt{data\_in} port to all 3 engines. Finally, 3 independent 32-bit fixed-point adders are responsible for adding the generated dot products to the cascaded input from the previous tensor block. As seen in Fig. \ref{fig_tensor_block_diagram}, starting from Tensor block 1, accumulation results are propagated along a Tensor block chain through hardwired connections between a block's \texttt{cascade\_data\_out} port and the following block's \texttt{cascade\_data\_in} port. The maximum chain length is 36. The outputs of final tensor block in the chain are exposed through the 3 25-bit wide \texttt{data\_out} ports. 

We use two modes for loading weights into the Tensor blocks. The first is the parallel load mode, where the 80-bit data\_in port is used to load the weights into the buffers. No computation can take place during this operating mode. The second is the cascade mode, where the weights are propagated along a chain from the \texttt{cascade\_weight\_out} port of one block to the \texttt{cascade\_weight\_out} port of the next. In our case, the first Tensor block in a cascade chain is sacrificed and works in the parallel load mode, serving as a chain's point of entry for the weights. Subsequent blocks in the chain receive their weights in a cascade mode. In both modes, 3 clock cycles are needed to load weights into all 3 buffers. Loading weights can be overlapped with dot product operations to hide the loading latency. While buffer 0 is being multiplied with a set of inputs, buffer 1 can be loaded. It becomes clear that the longer the length of the cascade chain, the higher the weight loading latency. Since, the maximum chain length is 36, then the maximum latency is 108 cycles. However, each weight can get multiplied with a large amount of inputs in a GEMM operation, more specifically equal to N. If the native N size is at least 108, which is a reasonable assumption, then the weight loading can be fully overlapped.

\subsection{GEMM accelerator architecture}
\textcolor{red}{Explain a couple things about architecture before starting with the parameters...} We define 4 different architecture parameters for implementing a GEMM engine on Stratix 10 NX. 
\begin{itemize}
    \item \textit{\arraylength}: Length of a cascade chain. Less than or equal to 36. We refer to this as an array of cascaded tensor blocks.
    \item \textit{\Kexpansion}: Set of arrays that work in parallel across the K dimension. The \texttt{data\_out} outputs of all these arrays are grouped and fed into an adder tree. We refer to this array set as a column block.
    \item \textit{\Nexpansion}: Set of column blocks that contain the same weights, but get multiplied with different columns of the input matrix. Allows exploiting parallelism across the N dimension. We refer to the set of column blocks as a row block.
    \item \textit{\Mexpansion}: Total number of row blocks that allow parallelism across the M dimension.
\end{itemize}
These parameters are illustrated in Figure \ref{fig_tb_layout}, where the data processed by each tensor block is represented with a combination of a shape, a color and a number. The shape represents the weights of the weight matrix that get stored in each tensor block. Each shape actually represents a block of 3 rows and 10 columns. The color represents the corresponding data from the input matrix that get multiplied with the stored weights of each tensor block. Each entry in the input matrix is actually a block of 10 rows and 1 column. Finally, the number in each entry of the input matrix indicates the clock cycle that an input block gets multiplied with the corresponding weights in the tensor block. We observe that each tensor block in an array holds different weights and gets multiplied with different inputs. However, each tensor block starts processing data two cycles after its preceding tensor block, as it has to wait for its \texttt{cascade\_data\_out} to be ready, as shown in Fig. \ref{fig_tensor_block_diagram}. Different arrays in a column block hold separate weights and process separate inputs, but have identical times. Column blocks of the same row block hold the same weights, but get multiplied with different inputs. Finally, different row blocks contain different weights, but get multiplied with the same inputs.

Below we list several considerations regarding each of the 4 parameters, along with some constraints they introduce.
\begin{itemize}
    \item \textit{\arraylength}: The maximum chain length, as mentioned, is 36. Moreover, the Tensor blocks are packed in groups of 36 along a column in the FPGA chip. There is no cascade connection possible between the last and the first tensor blocks of two subsequent groups in an  FPGA column. As a result, the chain length must be a factor of 36 in order to avoid fragmentation during placement of a design with a large utilization of Tensor blocks. Good chain lengths are 36, 18, 12 and 9. Low chain lengths lead to more wasted Tensor blocks for cascading weights, but offer a higher flexibility in supported native matrix sizes. Large chain lengths lead to a longer weight loading latency, but a higher peak throughput.
    \item \textit{\Kexpansion}: If a maximum chain length of 36 is used, then a 350-column wide block of weights is stored in an array. When the reduction dimension (K) is large, one can either tile through blocks of size 350, or increase the block size by adding more arrays in a column block. The second option allows more flexibility in utilizing a large number of Tensor blocks, while keeping the signal fanout low. The outputs of all the chains in a column block are gathered in an adder tree, the output of which is fed into an accumulator placed closed to the output buffer. These adders are implemented in soft logic.
    \item \textit{\Nexpansion}: If this parameter is set to 1, one must use a very large \Mexpansion to further increase the tensor block utilization. However, this greatly increases the fanout of all the data inputs and leads to high routing congestion. \Nexpansion allows us to leverage more parallelism by broadcasting weights along with data. This is great for routability, since each array only has only one 80-bit wide input for weights, while the number of 80-bit wire connections required for input data is equal to $\arraylength[~] - 1$. \textit{\Nexpansion[~]} introduces a constraint on the native N dimension of the accelerator. For example, assume a row block with 3 column blocks and arrays of 4 tensor blocks each. A total of $4\times3=12$ cycles are needed to load the weights on each column block's array. In order to fully overlap weight loading latency with computation, each of these weights must be multiplied with at least 12 inputs. As a result, N must be large enough to satisfy this for all column blocks. In this case, N must be $>= 36$. 
    \item \textit{\Mexpansion}: This parameter is essential in leveraging parallelism across the M dimension as well. However, as mentioned, the higher the \textit{\Mexpansion}, the higher the fanout of the data signals. As a result, greatly increasing the number of row blocks can lead to high routing congestion, harming attainable clock frequency and, ultimately, performance.
\end{itemize}

\subsection{Memory architecture}
It becomes clear that, when a large number of tensor blocks are used, a high SRAM bandwidth is needed to feed the weights and inputs and to keep them busy. One must carefully design the BRAM architecture to enable high performance and maximize BRAM utilization. Similarly to our Versal design, we maintain separate buffers for weight, input and output data. We are using double-buffering in all our designs. The load/store units perform read and write operations on output buffers and write-only operations on the weight and input buffers. The computation logic performs read and write operations on the output buffers and read-only operations on the input buffers. All the BRAMs in our design are configured in Simple Dual Port mode. For the weight and input BRAMs, the compute and load/store units have their own dedicated port for reading and writing, respectively. For double-buffering, we simply double the depth of these BRAMs. For the output BRAMs, since both the compute and the load/store units do read and write operations, we split output data into two separate buffers of equal size and add a standard interconnect logic to implement double-buffering.

Below we describe the architecture of the input, weight and output BRAMs in more detail.
\begin{itemize}
    \item \textit{Input data}: As we see in Fig.~\ref{fig_tb_layout}, each tensor block in an array (except for the first one that operates in parallel loading mode), receives separate inputs in each cycle. Similarly, all arrays across a column block and all column blocks along a row block require different inputs. The total number \textit{IBRAM} of required input data BRAMs is:
    \begin{equation}
        IBRAM = \textit{\arraylength} \times \textit{\Kexpansion} \times \textit{\Nexpansion}
    \end{equation}
    Each BRAM has a 80-bit wide port and a depth that is determined by the native K by N dimensions. Since the M20K blocks can provide 40-bit wide ports in Simple Dual Port mode, two M20K blocks are required at minimum to implement an input BRAM. As a result, careful selection of the native K by N dimensions is required to maximize the utilization of the used M20K blocks. We will investigate this matter further in section \ref{sec:Results}.
    \item \textit{Weight data}: Looking at Fig.~\ref{fig_tb_layout}, we see that a separate weight input must be fed to each array in a column block and across different row blocks. The total number \textit{WBRAM} of required weight BRAMs is:
    \begin{equation}
        WBRAM = \textit{\Kexpansion} \times \textit{\Mexpansion}
    \end{equation}
    Typically, WBRAM is much smaller than IBRAM and each weight BRAM has a larger depth than an input BRAM, so it is easier to efficiently utilize the weight BRAMs, by properly selecting the native M size.
    \item \textit{Output data}: Looking at Fig.~\ref{fig_tb_layout}, we see that a separate output is separated by each column block. Additionally, since each Tensor block has 3 dot product engines, each column block actually generates 3 outputs per clock cycles. The total number \textit{OBRAM} of output BRAMs is:
    \begin{equation}
        OBRAM = \textit{\Mexpansion} \times \textit{\Nexpansion} \times 2
    \end{equation}
    We multiply by 2 for double-buffering. The \texttt{data\_out} ports of each chain are 25-bit wide each. The accumulation on the output BRAMs is configurable by the user, ranging from 25 to 32 bits. However, we have 3 such outputs per array. As a result, we can either have \textit{OBRAM} total BRAMs with 80-bit wide ports, where all 3 outputs of a chain are concatenated and stored together, or $3 \times \textit{OBRAM}$ total BRAMs with port widths in the range of 25-32. The first option yields slightly better BRAM utilization (up to 50\% in most cases), but the second option yields higher attainable frequency and, thus, performance, so we chose this implementation for our analysis. Our tool supports generation of both designs.
\end{itemize}

\subsection{Optimization strategies}

We implement additional, standard optimizations to cut down the design's critical paths, such as replication of control logic and insertion of pipeline stages along the data and address datapaths. \textcolor{red}{Talk about pipeline stages in more detail here...}. Finally, we also explored the addition of \textcolor{red}{daisy chains of the input data in order to cut down the routing congestion caused by the input data fanout.}


We developed a tool that automatically generates the aforementioned architecture's Verilog code, including the tensor block layout, memory and all interconnect logic. The input configurations to the tool are the four architecture parameters, the native M, N and K dimensions, the output BRAM specification and the number of pipeline stages for address and data.

\subsection{Accelerator Latency}

Below we present the formula to accurately calculate the latency (in clock cycles) to fully process an MxKxN native block using the aforementioned architecture.

The time $t_{load}$ to load the weights into the arrays and the time $t_{prop}$ to propagate an accumulation from the start to the end of an array are both determined by the \arraylength:
\begin{equation}
t_{load} = \arraylength\times3, t_{prop} = (\arraylength-1)\times2
\label{eq_load_prop_times}
\end{equation}
\noindent Assuming adder trees comprising adders with 1-cycle latency, the latency $t_{adder}$ of an adder tree is:
\begin{equation}
t_{adder} = \log_2 (\Kexpansion)
\label{eq_adder_tree_time}
\end{equation}
\noindent After these initial latencies, a new output is generated every clock cycle. As mentioned earlier, given enough input matrix columns, the weight loading latency can be fully overlapped. The time $t_{N}$ to iterate through all the columns of the input matrix (N) depends on \textit{\Nexpansion}:
\begin{equation}
t_{N} = \frac{N}{\Nexpansion}
\label{eq_N_time}
\end{equation}
\noindent The total number of elements along the K dimension $D_K$ and the number of rows of a weight matrix $R_W$ that get processed every time are equal to:
\begin{equation}
D_{K} = (\arraylength-1)\times\Kexpansion\times10
\label{eq_data_processed}
\end{equation}
\begin{equation}
R_W = \Mexpansion\times3
\label{eq_rows_processed}
\end{equation}
\noindent Finally, the total number of cycles $t_{total}$ to fully process an MxKxN GEMM is:
\begin{equation}
t_{total} = t_{load} + t_{prop} + t_{adder} + \frac{M\times K}{D_{K}\times R_W}\times t_N
\label{eq_total_time}
\end{equation}

==> Versal_AI_Engines/Versal.tex <==






